Language Models Enable Simple Systems for Generating Structured Views of Heterogeneous Data Lakes

A long standing goal of the data management community is to develop general, automated systems that ingest semi-structured documents and output queryable tables without human effort or domain specific customization. Given the sheer variety of potential documents, state-of-the art systems make simplifying assumptions and use domain specific training. In this work, we ask whether we can maintain generality by using large language models (LLMs). LLMs, which are pretrained on broad data, can perform diverse downstream tasks simply conditioned on natural language task descriptions. We propose and evaluate EVAPORATE, a simple, prototype system powered by LLMs. We identify two fundamentally different strategies for implementing this system: prompt the LLM to directly extract values from documents or prompt the LLM to synthesize code that performs the extraction. Our evaluations show a cost-quality tradeoff between these two approaches. Code synthesis is cheap, but far less accurate than directly processing each document with the LLM. To improve quality while maintaining low cost, we propose an extended code synthesis implementation, EVAPORATE-CODE+, which achieves better quality than direct extraction. Our key insight is to generate many candidate functions and ensemble their extractions using weak supervision. EVAPORATE-CODE+ not only outperforms the state-of-the art systems, but does so using a sublinear pass over the documents with the LLM. This equates to a 110x reduction in the number of tokens the LLM needs to process, averaged across 16 real-world evaluation settings of 10k documents each.

==> sections/aggregation.tex <==
\begin{algorithm}[t]
\caption{\systemnamea{}}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Documents $\mathcal{D}$, candidate functions $F$, FM $\mathcal{F}$. \newline \textbf{Output:} Predicted extractions ${\hat{y}i, ..., \hat{y}n}$ for documents.
\STATE \textbf{Collect sample predictions} Sample $\mathcal{D}_{eval} \subset \mathcal{D}$ and apply the functions $f_j \in F$ and FM $\mathcal{F}$ to obtain $\hat{y}_{ij}$ and $\hat{y}_{i\mathcal{F}}$ for document $d_i$.
\STATE \textbf{Handle abstensions}: For empty $\hat{y}_{ij}$, we need to determine if they represent ``Function Abstensions'' or predictions that $d_i$ has ``No Attribute Value''. To decide between cases, use $\mathcal{F}$: compute $e$ as the fraction of documents $d_i \in \mathcal{D}{eval}$ with non-empty: $\hat{y}_{i\mathcal{F}}$
% fraction $e$ across 
\STATE \textbf{Score functions}: Compute a score $s_j$ for $f_{j}$ using metric function $m(\cdot)$ based on $e$. \\
    \textbf{if $e > \tau$ then} \\  \setlength\parindent{24pt} $s_j = \sum_{i=1}^{i=n} m(\hat{y}_{i\mathcal{F}}, \hat{y}_{ij})$, where $\hat{y}_{ij}$ is non-empty. \\
    \noindent \textbf{else} \\
    \setlength\parindent{24pt} $s_j = \sum_{i=1}^{i=n} m(\hat{y}_{i\mathcal{F}}, \hat{y}_{ij})$ \\
\STATE \textbf{Filter low-quality functions} Remove $f_j \in F$ with $s_j \leq 0.5$ to create $F'$.
\STATE \textbf{Collect votes} 
Apply $f \in F'$ to all $d_i \in \mathcal{D}$ to collect ``votes'' for the attribute-value in $d_i$. Post-process empty-votes as abstensions or ``No Attribute'' predictions depending on $e$. 
% \hat{y}{ij}$ for $f_j \in \mathcal{E}{final}$, $d_i \in \mathcal{D}$.
\STATE \textbf{Aggregation} Use weak-supervision to obtain the final prediction $\hat{y}_i$ given the function votes $\{\hat{y}_{ij}|f_j \in F'\}$.
\end{algorithmic}
\label{alg:approach}
\end{algorithm}


\subsubsection{Unsupervised Function Verification} 
\label{sec:approach_alg}
We discuss how \systemname{} uses the sets of candidate functions synthesized for each attribute to provide the final predictions for the documents' attribute values. 

\paragraph{Background: Methods for Unsupervised Aggregation}
Because we lack ground truth labels in our setting, it is not possible to directly evaluate the quality of the candidate functions. A popular unsupervised aggregation strategy is to take the Majority Vote (MV) across function outputs \cite{wang2022selfconsistency}. Formally, MV treats the functions as independent of one another and assigns equal weight to all function outputs. However, as shown in Figure \ref{fig:best_extractor_split}, the functions are not of equal quality. Therefore, \systemname{} uses weak supervision (WS), a popular standard statistical framework for modeling the accuracies and correlations between noisy sources of information without any labeled data \cite{ratner2017snorkel, fu2020fast}. WS is widely used in industry \cite{ratner2017snorkel}. 

Unfortunately, the standard programmatic WS setup makes several assumptions that do not apply in our setting. The gap arises because the standard programmatic WS setup assumes \textit{human-designed} functions that output standardized classes for classification. In contrast, the functions in our setting are \textit{machine-generated} functions that output non-standardized extracted text. Our setting violates the following assumptions of the existing WS setting:

\begin{enumerate}
    \item \textbf{Assumption 1: Functions will abstain on examples where they do not apply \cite{ratner2017snorkel, fu2020fast}.} WS is able to exploit high-precision functions that may not have high recall. When humans design functions, they typically specify conditions under which the function should abstain (or do not apply). 
    However, it is challenging to generate functions with this advanced logic.
    As a result, the machine-generated functions from our prompts \textit{always} provide some output. This is particularly important when the function is not able to extract a value from a document, which can either be because the attribute does not exist in the document (``No Attribute Value'', e.g. a Wikipedia page may be missing a college attribute since historically, not all basketball players have attended college) or because the attribute exists but the function does not apply to this specific instance (``Function Abstension'', e.g. the  \verb|product code| attribute value starts with a lower-case ``k'' in the minority of FDA reports and capital ``K'' in the majority. \systemname{} generates functions for both cases, which output the \verb|product code| on relevant documents, and empty-strings otherwise.). If we cannot distinguish between cases, we will not be able to exploit high-precision / low-recall functions in our setting.
    \item \textbf{Assumption 2: Functions are correlated with the ground truth label $y$ at better than random performance \cite{ratner2017snorkel, fu2020fast}}. While this is reasonable when functions are human-designed, \systemname{} uses machine-generated functions. We find that 51\% of generated functions are below 50 Text-F1 (Figure \ref{fig:best_extractor_split}). 
    \item \textbf{Assumption 3: Weak supervision is typically applied to tasks with well-defined classes in a classification setting \cite{ratner2017snorkel, fu2020fast}.}  In our case, the output of the functions are extracted text, and thus there is a virtually unconstrained output space of possible extractions that vary from document to document (i.e. the value for the \verb|place of birth| attribute in different NBA player pages will differ). The \textit{number} of unique extractions collected by the functions can also differ across documents.
\end{enumerate}

 \begin{figure}
    \centering
\includegraphics[width=0.7\columnwidth]{figures/function_quality.png}
    % \vspace{-4mm}
    \caption[width=\columnwidth]{Across the gold attributes and settings, we report the estimated quality of the generated extraction functions.}
    \label{fig:best_extractor_split}
    % \vspace{-3mm}
\end{figure}

We propose the following approach to be able to leverage WS. Let $D_{eval}$ be a small sample of documents from the data lake $\mathcal{D}$. We have the set of generated functions $F$ and FM $\mathcal{F}$.

\paragraph{Identifying function abstentions.} Our objective is to estimate the probability that an empty output from a function is an abstension. We propose to measure the fraction $e$ of the $D_{eval}$ documents for which $\mathcal{F}$ extracts a value. Intuitively, when $e$ is high, this suggests the attribute appears in a large fraction of documents, so we should assume functions are abstaining when they output empty values. When $e$ is low, the attribute appears in very few documents, so we should assume the functions are outputting empty values. Thus, we can use $e$ to guide both our function evaluation and downstream aggregation. Note that it is possible for $\mathcal{F}$ to abstain or hallucinate values when they do not exist in the document, affecting the estimate of $e$.

\paragraph{Filtering functions with worse than random performance.} 
One key observation is that we can utilize the high-quality FM $\mathcal{F}$ on a small set of documents $D_{eval}$ (e.g. we use $|D_{eval}| \leq 10$). In Table \ref{tab:fm_closedie_baseline}, we validate that FMs are able to generate high-quality extractions for a wide range of attributes and document formats. We can leverage these as a high-quality estimate of the ground truth extractions for those documents.
We compute a score $s_j$ by comparing the outputs of function $f_j(\cdot)$ against the outputs of $\mathcal{F}$ on document $d_i \in \mathcal{D}_{eval}$. If we are in the low $e$ regime, we should evaluate the outputs on all $d \in \mathcal{D}_{eval}$. If we are in the high $e$ regime, we should evaluate the outputs on only the $d \in \mathcal{D}_{eval}$ for which the function extracted a value. We finally filter any function $f_j$ with scores $s_j \leq 0.5$, where $0.5$ derives from the typical WS assumptions \cite{ratner2017snorkel, varma2018snuba, fu2020fast}.



\paragraph{Handling extractions with unconstrained output spaces.} The $k$ generated functions can produce $[0..k]$ unique prediction votes for a single unlabeled document $d_i$, and the number of unique votes can differ from document $d_i$ to $d_j$. We therefore, for each $d_i \in \mathcal{D}$, bucket the unique votes and take the $b$ buckets representing the most frequently occurring votes. The votes for functions that outputted values outside the top-$b$ are marked as abstensions. If the number of unique votes is $< b$, placeholder values are inserted into the top-$b$. Finally, as the ``classes'' differ across documents, we introduce a constraint to the objective function encouraging the class-conditional accuracies to be equal.  

After addressing these assumptions, we can leverage prior approaches to aggregate the noisy extractions from the function candidates into higher quality extractions as in \cite{ratner2017snorkel, arora2022ama}. Under WS, the output of each function is viewed as a ``vote'' for the true label and the objective is to construct a latent graphical model to account for the varied accuracies and correlations amongst the functions, without access to any labeled data. Our method for aggregation is summarized in Algorithm \ref{alg:approach}.

\subsubsection{Unsupervised Schema Verification.}
Finally, after extracting values with the ensembled functions, we validate the by asking the LLM whether the extracted values are congruent with the attribute's name. For example, we pose the question, "Can 1993 be a position in a database table of NBA players?". We do this for a small sample of records (\textit{e.g.} 5). If LLM responds "No" for the entire sample values, the attribute is removed from the schema. Full prompts for this step are included in section \cref{app:schema-valid}.



==> sections/approach.tex <==
\label{sec:approach}

\vspace{-2mm}
\subsubsection{Schema Synthesis }
\label{sec:approach_schema}


 \systemname{} begins by prompting an LLM to identify attributes $A = \{a_1, a_2, ... a_m\}$ for the output table's schema. 
 
\paragraph{Generating candidate attributes} Concretely, we sample a set $\tilde{D}$ of $k << n$ documents from $D$. For each, we prompt the LLM to extract the most useful attributes from the document as in \systemnamea{}. Recall this yields a set of attributes ranked by how frequently they were extracted across documents. Because the LLM can hallucinate or inconsistently reword attributes as identified in Section \ref{sec:approach-integrated}, we filter out any attributes that were not explicitly mentioned in any of the documents. This ensures provenance in schema identification.
 
\paragraph{Re-ranking candidate attributes}  Because \systemname{} now identifies the attributes from a small set documents, we observe that \systemname{}'s ranking is noisier than when every document was processed in \systemnamea{}, i.e. an important attribute may be selected few times amongst the $k$ documents due to sampling errors. To address this, we introduce a new prompting step in which we include the union of extracted attributes and instruct the LLM to identify the most useful attributes (Appendix \ref{sec:microprompts}). High quality on this task reflects the powerful reasoning capabilities of recent LLMs. Finally, the frequency-based rank is upweighted by a constant multiplicative factor if the attribute is included in the LLM output.




 \begin{figure}
    \centering
\includegraphics[width=\columnwidth]{figures/crossinglines.png}
    \vspace{-4mm}
    \caption[width=\columnwidth]{Tradeoffs between processing the data lake with the LLM (End-to-End) vs. with our proposed system (\systemname{}). For small data lakes and large numbers of attributes, processing with the LLM is sufficient. As the data lake grows and attributes of interest become concise, \systemname{} is orders of magnitude more efficient. Left is evaluated at 10 attributes, Right at 10K documents. Assumes 10K tokens per document.}
    \label{fig:crossinglines}
\end{figure}


\subsubsection{Function Synthesis} 
\label{sec:approach_extract}
 
Given the attributes $A = \{a_1, a_2 ... a_m\}$, the objective of \systemname{}'s second phase is to extract the values of the attributes for each document $d_i \in D$.   
Our key insight, as discussed, is that attribute-values are expressed in similar ways from document to document. To exploit this, instead of processing every document with the LLM to extract values for attribute $a_i$, we propose to use the LLM to \textit{generate code} that can then be reused to process many documents. 

\paragraph{Function synthesis prompts} Figure \ref{fig:function_prompts} shows an \systemname{} function generation prompt. The in-context examples show pairs of text snippets and functions to extract an attribute of interest. \systemname{} searches the data lake via a simple keyword search for document portions that mention $a_i$, and includes this in the prompt. \systemname{} synthesizes functions for attributes following the rank order of attributes derived in the schema identification step. This means that values the most relevant (and frequent) attributes as determined by \systemname{} are extracted first, and the user can stop the synthesis when desired.


\paragraph{Improving the diversity of synthesized functions}  We find that the quality of LLM generated functions varies significantly depending on the document chunk and in-context examples used in the prompts. To address the variability in function quality, we adopt the strategy we previously proposed in \citet{arora2022ama}. This strategy curates multiple diverse prompts \textit{that follow the same template}  (i.e. multiple function generation prompts in the style of Figure \ref{fig:function_prompts}) and prompts the LLM with each in turn \textit{per inference example} (i.e. data lake documents) to produce a diverse set of \textit{function candidates} $F = \{f_1, f_2, ... f_{k}\}$. 

Concretely, we curate two function generation prompts $P_A$ and $P_B$ (both included in Appendix \ref{app:fn_gen}). $P_A$ includes no in-context examples, only a task description that encourages the LLM to use regular expressions. $P_B$ includes two in-context examples along with the task description that encourages the LLM to import and use any Python library of choice. We find that neither consistently outperforms the other. $P_A$ produces higher quality functions on $69\%$, $45\%$, $60\%$, $91\%$, and $31\%$ of attributes on the 8 SWDE Movie, 5 SWDE University, FDA reports, Enron and Wikipedia player pages settings respectively. Writing a single ``perfect'' prompt that performs well across all documents can be challenging and asking the LLM to complete the task in multiple ways helps.


\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/function_generation_prompt.pdf}
    \caption[width=\columnwidth]{Example prompt for generating functions to perform  information extraction. The prompt includes two generic in-context examples.}
    \label{fig:function_prompts}
\vspace{-3mm}
\end{figure}







==> sections/fm_background.tex <==
\label{sec:llm-background}

In this section, we provide background on \textit{large language models} (LLMs), which are central to our work.

\begin{definition}[Large Language Model]
A machine learning model, $\mathcal{F}$, trained on a self-supervised task (\textit{e.g.} next word prediction) over a massive corpus of text~\cite{gao2021pile}. Language models can be used to generate new text based on provided context. For example:
$$
\mathcal{F}(\text{All that glitters }) \rightarrow \text{is not gold.}
$$
\end{definition}

Numerous studies have demonstrated LLMs capable of solving new tasks without updating any model parameters, a phenomenon termed \textit{in-context learning}~\cite{brown2020language,agrawal2022clinicalie,narayan2022can}. 
Specifically, these studies show that when passed an appropriate description of the task, the model often generates text completing the task. 

\begin{definition}[Prompt]
A natural language task-specification used to elicit a particular generation from an LLM. Prompts often include demonstrations of the task.
For example, the prompt below elicits the translation of the word cheese into French: 
$$
\mathcal{F}(
\underbrace{\text{Translate. Eng: hello, Fr: bonjour; Eng: cheese, Fr: }}_{\mathclap{\textbf{Prompt}}}
) \rightarrow \underbrace{ \text{fromage}}_{\mathclap{\textbf{Generation}}}
$$
\end{definition}

Further examples of prompts used in this work are provided in \cref{fig:end2end,fig:function_prompts}.
 

==> sections/math_command.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm, amsthm, mathtools}
\newtheorem{proposition}{Proposition}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{observation}{Observation}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{assumption}{Assumption}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}[2]{\mathbb{E}_{#1}\left[#2\right]}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


\newcommand{\ind}[1]{\mathbbm{1}\left\{#1\right\}}
\newcommand{\D}[0]{\mathcal{D}}
\newcommand{\Dtest}[0]{\mathcal{D}_{\text{test}}}
\newcommand{\ntest}[0]{n_{\text{test}}}
\newcommand{\Y}[0]{\mathcal{Y}}

\newcommand{\yhat}[0]{\hat{y}}
\newcommand{\yama}[0]{\hat{y}_{\problemshortname}}

\newcommand{\phiws}[0]{\phi_{\text{WS}}}

\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;} 




==> sections/prompt_formats.tex <==
\section{Prompts}

\label{sec:microprompts}

Here we include all prompts used in the paper. \\

\subsection{End-to-end prompt} 
\label{sec:prompt-1}
The prompt that instructs the model to produce all useful attribute-value pairs mentioned in a ``chunk'' of document text is as follows. This prompt is used both as the end-to-end prompt in \systemnamea and for schema identification in \systemnameb and \systemnamec. The same prompt is applied to multiple chunks across multiple documents across our 16 evaluation settings, and contains generic in-context examples.

\begin{mdframed*}
% Input
\begin{codeframe}
\begin{lstlisting}
Sample text:
<tr class="mergedrow"><th scope="row" class="infobox-label"><div style="text-indent:-0.9em;margin-left:1.2em;font-weight:normal;"><a href="/wiki/Monarchy_of_Canada" title="Monarchy of Canada">Monarch</a> </div></th><td class="infobox-data"><a href="/wiki/Charles_III" title="Charles III">Charles III</a></td></tr>
<tr class="mergedrow"><th scope="row" class="infobox-label"><div style="text-indent:-0.9em;margin-left:1.2em;font-weight:normal;"><span class="nowrap"><a href="/wiki/Governor_General_of_Canada" title="Governor General of Canada">Governor General</a></span> </div></th><td class="infobox-data"><a href="/wiki/Mary_Simon" title="Mary Simon">Mary Simon</a></td></tr>
<b>Provinces and Territories</b class='navlinking countries'>
<ul>
<li>Saskatchewan</li>
<li>Manitoba</li>
<li>Ontario</li>
<li>Quebec</li>
<li>New Brunswick</li>
<li>Prince Edward Island</li>
<li>Nova Scotia</li>
<li>Newfoundland and Labrador</li>
<li>Yukon</li>
<li>Nunavut</li>
<li>Northwest Territories</li>
</ul>

Question: List all relevant attributes about 'Canada' that are exactly mentioned in this sample text if any.
Answer: 
- Monarch: Charles III
- Governor General: Mary Simon
- Provinces and Territories: Saskatchewan, Manitoba, Ontario, Quebec, New Brunswick, Prince Edward Island, Nova Scotia, Newfoundland and Labrador, Yukon, Nunavut, Northwest Territories

----

Sample text:
Patient birth date: 1990-01-01
Prescribed medication: aspirin, ibuprofen, acetaminophen
Prescribed dosage: 1 tablet, 2 tablets, 3 tablets
Doctor's name: Dr. Burns
Date of discharge: 2020-01-01
Hospital address: 123 Main Street, New York, NY 10001

Question: List all relevant attributes about 'medications' that are exactly mentioned in this sample text if any.
Answer: 
- Prescribed medication: aspirin, ibuprofen, acetaminophen
- Prescribed dosage: 1 tablet, 2 tablets, 3 tablets

----

Sample text:
{{chunk:}}

Question: List all relevant attributes about '{{topic:}}' that are exactly mentioned in this sample text if any. 
Answer:
\end{lstlisting}
\end{codeframe}
\end{mdframed*}

\subsection{Schema Re-ranking Prompt}
\label{sec:prompt-2}
This prompt is use to rerank the schema attributes identified by the prior schema identification prompt (Prompt \ref{sec:prompt-1}). This is useful to prioritize the attributes for which to generate extraction functions in the subsequent steps of \systemname{}.
\vspace{2mm}

\begin{mdframed*}
\begin{codeframe}
\begin{lstlisting}
Attributes:
{'name': 'Jessica', 'student major': 'Computer Science', 'liscense': 'accredited', 'college name': 'University of Michigan', ''GPA': '3.9', 'student email': 'jess.at.umich.edu', 'rating': '42', 'title': 'details'}

List the most useful keys to include in a SQL database for "students", if any.
Answer: ['name', 'student major', 'college name', 'GPA', 'student email']

----

Attributes:
{{Identified Schema}}

List the most useful keys to include in a SQL database for {{database-topic}}, if any.
Answer:
\end{lstlisting}
\end{codeframe}
\end{mdframed*}

\subsection{Attribute Extraction Prompt} 
\label{sec:prompt-5}
The following prompt is used to directly extract a provided ``attribute'' value from the provided ``chunk'' of document text. This prompt is used for collecting the high-quality \textbf{FM} $\mathcal{F}$'s ``labels'' on $\mathcal{D}_{eval}$, against which the generated functions $f \in \mathcal{E}$ are scored. The same prompt is applied to multiple chunks across multiple documents across our 16 evaluation settings, and contains generic in-context examples.

\begin{mdframed*}
\begin{codeframe}
\begin{lstlisting}
Here is a file sample:

<th>Location</th>
<td><a href="/wiki/Cupertino">Cupertino</a>, <a href="/wiki/California">California</a>Since 1987</td>

Question: Return the full "location" span of this sample if it exists, otherwise output nothing. 
Answer: 
- Location: Cupertino, California Since 1987

----

Here is a file sample:

{{chunk:}}

Question: Return the full "{{attribute:}}" span of this sample if it exists, otherwise output nothing.
Answer:
\end{lstlisting}
\end{codeframe}

\end{mdframed*}

\subsection{Function Generation Prompts}
\label{app:fn_gen}
\label{sec:prompt-3}
We use two generic prompts for function-generation as follows. These prompts correspond to $P_A$ and $P_B$ described in the Section \ref{sec:approach_extract} micro-experiments. The prompts accept ``chunks'' of document text that need to be parsed, the ``attribute'' of interest, and the cleaned attribute name ``function field'' (i.e. because attributes with ``/'', ``-'', etc. will not compile).

\begin{mdframed*}
\begin{codeframe}
\begin{lstlisting}
Here is a sample of text:

{{chunk:}}


Question: Write a python function to extract the entire "{{attribute:}}" field from text, but not any other metadata. Return the result as a list.


import re

def get_{{function_field:}}_field(text: str):
    \"""
    Function to extract the "{{attribute:}} field". 
    \"""
\end{lstlisting}
\end{codeframe}
\end{mdframed*}

\label{sec:prompt-4}
\newline \newline The second prompt is:
\begin{mdframed*}
\begin{codeframe}
\begin{lstlisting}
Here is a file sample:

DESCRIPTION: This file answers the question, "How do I sort a dictionary by value?"
DATES MODIFIED: The file was modified on the following dates:
2009-03-05T00:49:05
2019-04-07T00:22:14
2011-11-20T04:21:49
USERS: The users who modified the file are:
Jeff Jacobs
Richard Smith
Julia D'Angelo
Rebecca Matthews
FILE TYPE: This is a text file.

Question: Write a python function called "get_dates_modified_field" to extract the "DATES MODIFIED" field from the text. Include any imports.

import re

def get_dates_modified_field(text: str):
    \"""
    Function to extract the dates modified.
    \"""
    parts= text.split("USERS")[0].split("DATES MODIFIED")[-1]
    pattern = r'\d{4}-\d{2}-\d{2}T\d{2}:\d{2}:\d{2}'
    return re.findall(pattern, text)

----

Here is a file sample:

<title>U.S. GDP Rose 2.9% in the Fourth Quarter After a Year of High Inflation - WSJ</title>
<meta property="og:url" content="https://www.wsj.com/articles/us-gdp-economic-growth-fourth-quarter-2022-11674683034"/>
<meta name="article.published" content="2023-01-26T10:30:00Z"/><meta itemProp="datePublished" content="2023-01-26T10:30:00Z"/>
<meta name="article.created" content="2023-01-26T10:30:00Z"/><meta itemProp="dateCreated" content="2023-01-26T10:30:00Z"/>
<meta name="dateLastPubbed" content="2023-01-31T19:17:00Z"/><meta name="author" content="Sarah Chaney Cambon"/>

Question: Write a python function called "get_date_published_field" to extract the "datePublished" field from the text. Include any imports.

from bs4 import BeautifulSoup

def get_date_published_field(text: str):
    \"""
    Function to extract the date published.
    \"""
    soup = BeautifulSoup(text, parser="html.parser")
    date_published_field = soup.find('meta', itemprop="datePublished")
    date_published_field = date_published_field['content']
    return date_published_field

----

Here is a sample of text:

{{chunk:}}

Question: Write a python function called "get_{{function_field:}}_field" to extract the "{{attribute:}}" field from the text. Include any imports.
\end{lstlisting}
\end{codeframe}
\end{mdframed*}

\subsection{Unsupervised Schema Validation Prompts}
\label{sec:prompt-6}
\label{app:schema-valid}
The following prompt is used to determine the validity of an attribute identified and extracted during \systemname{}'s OpenIE execution. We apply the prompt to a small sample of (e.g. 5) values extracted from the documents, in turn, for a particular ``attribute''. If the FM outputs ``No'' for all values in the sample, the entire attribute is discarded from \systemname{}
s outputted structured view. 

\begin{mdframed*}
\begin{codeframe}
\begin{lstlisting}
Question: Could "2014" be a "year" value in a "students" database?
Answer: Yes

----

Question: Could "cupcake" be a "occupation" value in a "employee" database?
Answer: No

----

Question: Could "''" be a "animal" value in a "zoo" database?
Answer: No

----

Question: Could "police officer" be a "occupation" value in a "employee" database?
Answer: Yes

----

Question: Could "{{value:}}" be a "{{attr_str:}}" value in a {{topic:}} database?
Answer:
\end{lstlisting}
\end{codeframe}
\end{mdframed*}

\subsection{Atomic Schema Cleaning Prompts}
The following prompts are used for atomic schema cleaning experiment in Section \ref{sec:schema_cleaning_extensions}. Note these prompts are not used in the main results, but only to demonstrate a potential system extension. This prompt is used for the expensive FM to decompose complex attributes and values into atomic attributes and values.

\begin{mdframed*}
\begin{codeframe}
\begin{lstlisting}
Extract one or more atomic schemas and values from the given schemas and values as a JSON list of pairs.

Schema: Spouse
Value: Michelle Robinson (m. 1992)

Atomic schemas and values: [["Spouse Name", "Michelle Robinson"], ["Married Year", 1992]]

---

Schema: In office
Value: January 8, 1997 - November 4, 2004

Atomic schemas and values: [["In Office Start Year", "January 8, 1997"], ["In Office End Year", "November 4, 20024"]]

---

Schema: Gini (2020)
Value: 46.9

Atomic schemas and values: [["Gini 2020", "46.9"]]

---

Schema: Countries
Value: United States (29 teams)\n Canada (1 team)

Atomic schemas and values: [["Countries", ["United States (29 teams)", "Canada (1 team)"]]]

---

Schema: {{complex_attribute:}}
Value: {{complex_value:}}

Atomic schemas and values:
\end{lstlisting}
\end{codeframe}
\end{mdframed*}


The following prompt is used to prompt the smaller, inexpensive FM to extract the cleaned value from the complex value given the cleaned attribute and a one-shot demonstration from the expensive FM for atomic schema cleaning in Section \ref{sec:schema_cleaning_extensions}.


\begin{mdframed*}
\begin{codeframe}
\begin{lstlisting}
Extract the attribute from the context.

Context: {{complex_attribute_example:}}: {{complex_extraction_example:}}
Attribute: {{cleaned_attribute_example:}}
Value: {{cleaned_value_example:}}

---

Context: {{complex_attribute:}}: {{complex_extraction:}}
Attribute: {{cleaned_attribute:}}
Value:
\end{lstlisting}
\end{codeframe}
\end{mdframed*}

\subsection{Domain Specific Prompts}
\label{sec:prompt-dom}
\edit{The following prompt for schema identification is used for the domain specific prompts experiment in Section \ref{sec:domain-specific}, to demonstrate an avenue for further improving system quality. Note the prompt is not used in the main results, but only to demonstrate a potential system extension. }
\begin{mdframed*}
\begin{codeframe}
\begin{lstlisting}
f"""Sample text:
<span>Total Ratings: 1</span></div>
<div id="local-nav">
<ul>
<li><a href="overview">Overview</a></li>
<li><a href="awards">Awards</a></li>
<li><a href="review">Review</a></li>
</ul>
<br class="clear"/>
</div>
<!-- 4831 2010-11-14 01:17:42 -->
<!-- start details -->
<div class="list-listing details">
<h2>Movie Details:</h2>
<!-- Left column -->
<ul>
<li>Director: <span><a href="/person/86860/Valentine-Davies/details" title="Biography for director Valentine Davies">Valentine Davies</a></span></li>
<li>Produced By: <span>Universal</span></li>

Question: List all relevant attributes about 'motion pictures, movies' that are exactly mentioned in this sample text if any. 
Answer:
- Total Ratings: 1
- Director: Valentine-Davies
- Produced By: Universal

----

Sample text:
<li>Year: <span>2005</span></li>
<li>Run Time: <span>90 minutes</span></li>
<li>Country: <span>USA</span></li>
<li>Language: <span>English</span></li>
</ul>
<!-- Right column -->
<ul>
<li>MPAA Rating: <span>PG (for some brief language and suggestive humor)</span></li>
<li>Category: <span>Animated</span></li>
<li>Genre/Type: <span>Children's/Family</span></li>
</ul>
</div>
<hr/> <!-- required -->
<!-- start synopsis -->
<div id="synopsis">

Question: List all relevant attributes about 'motion pictures, movies' that are exactly mentioned in this sample text if any. 
Answer:
- Year: 2005
- Run Time: 90 minutes
- Country: USA
- Language: English
- MPAA Rating: PG (for some brief language and suggestive humor)
- Category: Animated
- Genre/Type: Children's/Family

----

Sample text:
{{chunk:}}

Question: List all relevant attributes about '{{topic:}}' that are exactly mentioned in this sample text if any. 
Answer:"""
\end{lstlisting}
\end{codeframe}
\end{mdframed*}

==> tables/fm_baseline.tex <==
\begin{table}[t]
    \centering
    \resizebox{0.48\textwidth}{!}{\renewcommand{\arraystretch}{0.98}
    \begin{tabular}{lccc|cc}
     \toprule
       \multirow{2}{*}{Source (Format)}  &  
       \multicolumn{3}{p{2.5cm}}{\centering \textsc{Quality}} & \multicolumn{2}{p{3cm}}{\centering \textsc{Cost / 10k Documents}} \\   & 
      \emph{R}  &   \emph{P} & \emph{F1}  & \emph{Tokens (M)} & \emph{Dollars (\$)}\\
    \midrule
     Enron Emails (\textsc{TXT}) & 85.8 & 96.6 & 90.9 &  21.2  & 425   \\
     FDA (\textsc{TXT})          & 39.2 & 63.9 & 48.6 & 145.6  & 2,900 \\
     Wiki NBA (\textsc{HTML})    & 40.7 & 52.7 & 45.9 & 650.1  & 13,000\\
     SWDE Movies (\textsc{HTML}) & 34.3  & 47.1 & 37.4 & 282.9 & 5,660 \\
     SWDE University (\textsc{HTML})  & 50.2 & 66.3 & 54.4 & 190.1 & 3,800 \\ 
     \hline
     \textbf{Average}  & \textbf{50.0} & \textbf{65.3} & \textbf{55.4} & \textbf{258.0} & \textbf{2,817} \\ 
     \bottomrule
    \end{tabular}}
\caption{Quality and cost achieved through directly prompting OpenAI's Text-Davinci-003 model to complete the end-to-end task of generating structured views from heterogeneous documents.}
\label{tab:end2end}
\end{table}




==> tables/gpt4.tex <==
\begin{table}[t]
    \centering
    \resizebox{0.48\textwidth}{!}{\renewcommand{\arraystretch}{0.98}
    \begin{tabular}{lccc|cc}
     \toprule
    Source (Format) &  R  &  P & Pair F1  & Base  & Ours\\
    \midrule
     Enron Emails (\textsc{TXT})      & 82.6 & 94.5 & 88.1 & 92.7  & 85.5 \\
     FDA (\textsc{TXT})               & 51.7 & 61.0 & 56.0 & 59.2 & 57.5 \\
     Wiki NBA (\textsc{HTML})         & 57.7 & 69.7 & 63.2  & 40.5 & 61.4\\
     SWDE Movie (\textsc{HTML})       & 50.0 & 62.3 & 54.8  & 35.1 & 54.9\\
     SWDE University (\textsc{HTML})  & 49.9 & 65.5 & 56.3  & 56.1 & 57.2 \\ 
     \midrule
     \textbf{Average} & \textbf{58.4} & \textbf{65.0} & \textbf{63.7} &  \textbf{56.7}&  \textbf{63.3} \\ 
     \bottomrule
    \end{tabular}}
\caption{OpenIE results as in Table \ref{tab:evaporate_openie} with OpenAI's GPT-4 FM as the high-quality FM.}
\label{tab:gpt4}
\end{table}


==> tables/notation.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{lp{6.4cm}}
\toprule
Notation & Definition \\
\midrule
$d \in \mathcal{D}$ & The set of $n$ documents in the data lake. \\
$a \in A$ & Attributes included in the output table. \\
\midrule
$d \in \tilde{\mathcal{D}}$ & Random sample of $k$ documents from $\mathcal{D}$ that are used for schema identification and function synthesis. \\
$p \in P$ & Number of unique prompts per prompt-template used to synthesize functions for function diversity. \\
$f \in F$ & Functions synthesized with the LM $\mathcal{F}$. \\
$d \in \tilde{\mathcal{D}}_{eval}$ & Random sample of $k$ documents from $\mathcal{D}$, distinct from $\tilde{\mathcal{D}}$, that are used to score the synthesized functions in Algorithm \ref{alg:approach}. \\
\midrule
$\mathcal{F}$ & The language model. \\
\bottomrule
\end{tabular}
\caption{User controls in \systemname{}.}
    \label{tab:notation}
\vspace{-3mm}
\end{center}
\end{table}

==> tables/open_models.tex <==
\begin{table}[t]
    \centering
    \resizebox{0.48\textwidth}{!}{\renewcommand{\arraystretch}{0.98}
    \begin{tabular}{lc|ccc}
     \toprule
       \multirow{2}{*}{Source (Format)}  &      \multicolumn{1}{p{1.4cm}}{\centering \textsc{ClosedIE}} &
       \multicolumn{3}{p{2.8cm}}{\centering \textsc{OpenIE}} \\
       &   \emph{F1}  &        
      \emph{R}  &   \emph{P} & \emph{F1}  \\
    \midrule
     Enron Emails (\textsc{TXT})      &  &  &  & \\
     FDA (\textsc{TXT})               &  &  &  & \\
     Wiki NBA (\textsc{HTML})         &  &  &  & \\
     SWDE Movie (\textsc{HTML})       &  &  &  & \\
     SWDE University (\textsc{HTML})  &  &  &  & \\ 
     \hline
     \textbf{Average}  & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\ 
     \bottomrule
    \end{tabular}}
\caption{}
\label{tab:open_models}
\end{table}

==> tables/slice_results.tex <==
\begin{table}[]
\begin{tabular}{l|cc|cc}
\toprule
\multirow{2}{*}{Source (\# data groups)} & \multicolumn{2}{c|}{\textsc{Popularity (F1)}} & \multicolumn{2}{c}{\textsc{Atomicity (F1)}}  \\
& \emph{Head}  & \emph{Tail}  & \emph{Atomic} & \emph{Complex} \\
\midrule
Wiki Players (1)       & 70.8 & 46.6 & 79.0   & 47.6 \\
Enron (1)              & 88.3 & 0.0  & 81.1   & 87.3 \\
FDA (1)                & 62.8 & -    & 60.9   & 51.6 \\
SWDE Movies (8)        & 58.0 & 23.9 & 57.4   & 51.9 \\
SWDE Universities (5)  & 85.7 & 0.0  & 77.6   & 47.5 \\
\midrule
 \textbf{Average}  & \textbf{73.1} & \textbf{17.6} & \textbf{71.2} & \textbf{57.4} \\ 
\bottomrule

\end{tabular}
\caption{Evaluation of \systemname{} by attribute slice. The \textit{head} slice includes attributes mentioned in >50\% of documents and less than 20 characters in length. The \textit{tail} slice includes attributes mentioned in <50\% of documents and less than 20 characters in length. Atomicity is defined by whether the average attribute value is longer or shorter than 20 characters in length. ``-'' indicates an empty slice.}
\label{tab:evaporate_slices}
\vspace{-5mm}
\end{table}

==> tables/synthetic_nba_tables.tex <==

\begin{table}[t]
    \centering
    \resizebox{0.48\textwidth}{!}{\renewcommand{\arraystretch}{0.98}
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    Source  & Number of Gold & Recall  & Recall \\
    (\# of documents) & Attributes ($|\mathcal{A}|$) & @$|\mathcal{A}|$ & @50\\
    \hline
    Wiki players (10) & 20 & \yell{75.0} & \yell{85.0} \\
    SWDE ESPN (10) & 21 &\yell{} & \yell{} \\
    SWDE IMDB (10) & 35 & \yell{}  & \yell{}  \\
    SWDE CollegeProwler (10) & 21 & \yell{}  & \yell{} \\
    Enron emails (10) & 18 & \yell{}  & \yell{} \\
    \hline
    \end{tabular}}
\caption{Schema identification quality.} 
\label{tab:synthetic_schema_id}
\end{table}


\begin{table}[t]
    \centering
    \resizebox{0.48\textwidth}{!}{\renewcommand{\arraystretch}{0.98}
    \begin{tabular}{|c|c|c|c|}
     \hline
     Source  & \# of Gold & Text & Tokens  \\
     (Total \# of Documents) & Attributes & F1 & Processed \\
    \hline
     Wiki players (100)  & 20 & \yell{69.4} & \yell{11.6 M} \\
    SWDE ESPN (434) & 21 &\yell{}  & \\
    SWDE IMDB (2000) & 35 & \yell{60.7}  &  \yell{142M} \\
    SWDE CollegeProwler (2000) & 21 & \yell{} & \\
    Enron emails (500K) & 18 & \yell{} &  \\
     \hline
    \end{tabular}}
\caption{Extraction quality in isolation.}
\label{tab:synthetic_info_extraction}
\end{table}

\begin{table}[t]
    \centering
    \resizebox{0.48\textwidth}{!}{\renewcommand{\arraystretch}{0.98}
    \begin{tabular}{|c|c|c|c|c|}
     \hline
     Source  & \# of Gold & Recall  & Precision & F1 \\
     (\# of documents) & Attributes & & & \\
    \hline
     Wiki players (10)  & 20 & \yell{} & \yell{} & \\
     SWDE ESPN (10) & 21 &\yell{} & \yell{} & \\
    SWDE IMDB (10) & 35 & \yell{}  & \yell{} & \\
    SWDE CollegeProwler (10) & 21 & \yell{}  & \yell{} & \\
    Enron emails (10) & 18 & \yell{} &  & \yell{} \\
     \hline
    \end{tabular}}
\caption{Schema cleaning in isolation.}
\label{tab:synthetic_schema_cleaning}
\end{table}


\begin{table}[t]
    \centering
    \resizebox{0.48\textwidth}{!}{\renewcommand{\arraystretch}{0.98}
    \begin{tabular}{|c|c|c|c|c|}
     \hline
     Source  & \# of Gold & Recall  & Precision & F1 \\
     (\# of documents) & Attributes & & & \\
    \hline
    Wiki players (10)  & 20 & \yell{8.8} & \yell{8.0} & \yell{8.4} \\
    SWDE ESPN (10) & 21 &\yell{} & \yell{} & \\
    SWDE IMDB (10) & 35 & \yell{15.2}  & \yell{13.0} & \yell{14.0} \\
    SWDE CollegeProwler (10) & 21 & \yell{}  & \yell{} & \\
    Enron emails (10) & 18 & \yell{} &  & \yell{} \\
     \hline
    \end{tabular}}
\caption{OpenIE quality as we increase the number of attributes to consider}
\label{tab:synthetic_openie}
\end{table}

